Pseudo-Trilateral Adversarial Training for Domain Adaptive Traversability Prediction

Traversability prediction is a fundamental perception capability for autonomous navigation. Deep neural networks (DNNs) have been widely used to predict traversability during the last decade. The performance of DNNs is significantly boosted by exploiting a large amount of data. However, the diversity of data in different domains imposes significant gaps in the prediction performance. In this work, we make efforts to reduce the gaps by proposing a novel pseudo-trilateral adversarial model that adopts a coarse-to-fine alignment (CALI) to perform unsupervised domain adaptation (UDA). Our aim is to transfer the perception model with high data efficiency, eliminate the prohibitively expensive data labeling, and improve the generalization capability during the adaptation from easy-to-access source domains to various challenging target domains. Existing UDA methods usually adopt a bilateral zero-sum game structure. We prove that our CALI model -- a pseudo-trilateral game structure is advantageous over existing bilateral game structures. This proposed work bridges theoretical analyses and algorithm designs, leading to an efficient UDA model with easy and stable training. We further develop a variant of CALI -- Informed CALI (ICALI), which is inspired by the recent success of mixup data augmentation techniques and mixes informative regions based on the results of CALI. This mixture step provides an explicit bridging between the two domains and exposes underperforming classes more during training. We show the superiorities of our proposed models over multiple baselines in several challenging domain adaptation setups. To further validate the effectiveness of our proposed models, we then combine our perception model with a visual planner to build a navigation system and show the high reliability of our model in complex natural environments.

==> log <==
135,146c135,150
< knowledge may impose limits that ultimately impede global optimality in a
< decentralized optimization problems.  This paper enhances a recent anytime
< optimal assignment method based on a task-swap mechanism by redesigning the
< algorithm to address task allocation problems in a decentralized fashion.  We
< propose a fully decentralized approach that allows local search processes to
< execute concurrently while minimizing interactions amongst the processes,
< needing neither global broadcast nor a multi-hop communication protocol.  The
< formulation is analyzed in a novel way using tools from group theory and the
< optimization duality theory to show that the convergence of local searching
< processes is related to a shortest path routing problem on a graph subject to
< the network topology.  Simulation results show that this fully decentralized
< method converges quickly while sacrificing little optimality.   
---
> knowledge may impose limits that run against global optimality in
> a decentralized optimization problem.
> This paper redesigns the task-swap mechanism recently introduced in an anytime assignment
> algorithm to tackle the problem of decentralized task allocation for large
> scale multi-robot systems.  We propose a fully decentralized approach that
> allows local search processes to execute concurrently while minimizing
> interactions amongst the processes, needing neither global broadcast nor a multi-hop
> communication protocol.
> The formulation is analyzed in a novel way using tools from 
> group theory and 
> the optimization duality theory to show that the 
> convergence of local searching processes is related to a shortest path
> routing problem on a graph subject to the network topology.  
> Simulation results show that this fully decentralized method converges quickly
> while sacrificing little optimality.   
> 
158,209c162,192
< Multi-robot task allocation or role assignment aims at finding the best
< matching between a set of robots and a set of tasks in order to optimize the
< team's performance.  It is among the most popular optimization formulations
< for coordination problems in multi-robot systems.  Solutions to general task
< allocation problems have also lead to specialized methods for applications of
< particular importance in robotics research, {\em e.g.}, by strategically
< setting the tasks as goal locations, the methods efficiently deploy robots as
< part of path planning~\citep{Turpin-RSS-13,turpin14ijrr} and formation control
< problems~\citep{michael08formation,Liu-DARS-12}.  Ultimately, a fundamental
< understanding of distributed assignment problems may also benefit other
< decentralized systems/missions such as automated transportation systems,
< large-scale swarm systems, unmanned planetary exploration, {\em etc}.
< % DAS: Personally, I think these shouldn't just be self citations.
< 
< A multi-robot team may adapt to circumstances, demonstrating fluid coordination
< by repeatedly allocating tasks to robots frequently.  While the
< classic optimal assignment (or weighted matching) algorithms seeks to reduce
< overall execution time and time complexity, the multi-robot task allocation
< setting has several features requiring special consideration.  
< For example, a single central controller that is relied upon to compute and
< broadcast the assignment solutions becomes a single point of failure for the
< robot team.  Instead, it is desirable that the computation should be carried
< out in a distributed way so that individual failures do not affect the whole
< system.  
< In addition to handling dynamics, emergencies, and unexpected contingencies
< smoothly, the responsiveness of the team depends on fast solution of the
< underlying assignment problem relative to the environment dynamics.  But many
< envisioned scenarios involve multiple robots being dispatched in a large
< workspace where each robot may only be able to communicate with comparatively
< few neighbors who are nearby. Unfortunately long message relays may hinder the
< system's responsiveness.  Also, the optimality of an assignment solution becomes
< moot if the system's state evolves so rapidly that the decision was made with
< outdated inputs.  Naturally both prohibitive communication delays and bandwidth
< limits may preclude the use of a {\em centralized} task allocation strategy.
< 
< The constraint of local communication may impact the final task allocation
< solution.  If each robot is permitted to share information with only neighbors
< in its vicinity and no multi-hop communications stratagem is employed, the
< resultant assignment solution may necessarily be suboptimal.  This is because a
< decentralized algorithm constrained by local communication  cannot guarantee
< that complete information will be aggregated without relaying messages, and the
< optimal solution may require the complete information.  Even for the simplest
< task allocation scenario involving one-to-one mapping of robots to tasks, it is
< still unclear what the best (potentially sub-optimal) assignment can be
< obtained subject to certain communication constraints.
< Nor has the converse question been addressed: given a requisite solution
< quality, what is the least interaction the agents will
< need to obtain a suitable solution?
< 
< In this paper, we explore decentralized task allocation methods where
< communication and computation are carried out concurrently in a spatially
< localized fashion so that the interaction between agents, in particular the
---
> Multi-robot task allocation or assignment aims at finding the best matching between a set of robots and a set of tasks in order to optimize the team's performance.
> It is one of the most popular optimization formulations for coordination problems in multi-robot systems. 
> Solutions to general task allocation problems have also lead to specialized methods for applications of particular importance in robotics research, {\em e.g.}, 
> by strategically setting the tasks as goal locations, the methods efficiently deploy robots as part of path planning~\citep{Turpin-RSS-13,turpin14ijrr} and formation control problems~\citep{michael08formation,Liu-DARS-12}.
> Ultimately, a fundamental understanding of distributed assignment problems may also benefit other decentralized systems/missions such as automated transportation systems, large-scale swarm systems, unmanned planetary exploration, {\em etc}.
> 
> A multi-robot team may adapt to circumstances and demonstrate fluid coordination by allocating tasks to robots repeatedly.
> While the classic optimal assignment (or weighted matching) algorithms seeks to
> reduce overall execution time and time complexity, the multi-robot task allocation setting has several features requiring special consideration.
> For example, a single central controller should not be relied upon 
> to compute and broadcast the assignment solutions but, instead, 
> computation should be carried out in a distributed way so that individual
> failures do not affect the whole system. 
> In addition to handling dynamics, emergencies, and unexpected contingencies smoothly, the responsiveness of the team depends on fast solution of the underlying
> assignment problem relative to the environment dynamics. 
> But many envisioned scenarios involve multiple robots being dispatched in a
> large workspace where each robot may only be able to communicate with
> comparatively few nearby neighbors.  Consequently, long message relays may
> hinder the system responsiveness.  Also, the optimality of an assignment
> solution becomes moot if the system's state evolves so rapidly that the
> decision was made with outdated inputs.
> Naturally both prohibitive communication delays and bandwidth limits may
> preclude the use of a {\em centralized} task allocation strategy.
> 
> The constraint of local communication may impact the final task allocation solution.
> Oftentimes, only suboptimal assignment solution can be obtained if each robot is allowed to share information with only neighbors in vicinity and if finite operations/time are allowed. This is because decentralized algorithms constrained by local communication usually rely on message broadcasting and relays and cannot guarantee to obtain the complete/global information required for computing the optimal solution. 
> However, even for the simplest task allocation scenario that makes one-to-one mapping assignment, it is still unclear that given certain ``level" of local interaction (e.g., a certain communication range, a certain execution period), what is the best assignment performance even if only sub-optimality can be reached.
> Conversely, given certain level of solution quality, what is the expected least amount of local interaction the agents will need.   
> 
> In this paper, we are motivated to explore decentralized task allocation methods where communication and computation are carried out in a spatially localized and
> concurrent fashion so that the interaction amongst agents, in particular the
211,226c194,209
< \footnotetext{$^\dagger$ The main algorithm was first presented in the 2014
< Robotics: Science and Systems conference~\citep{Liu-RSS-14}.} The work extends
< the recent task-swap based anytime optimal assignment
< method~\citep{liu-auro13}, which has a decentralized structure but may still
< entail multi-hop communication (global information).  This paper employs the
< same mechanism responsible for the atomic optimization step ({\em viz.} the
< task-swap), but loosens the global communication requirement in the search
< procedure that selects which step is performed.  Although the algorithm we
< present may produce suboptimal solutions, an inherent limitation arising from
< the fact that local information may be intrinsically inadequate, this new
< algorithm optimizes the search subject to the communication constraints and
< always produces the step with maximum convergence toward the optimal solution.
< Since local communication may impose limits that hinder global optimality, we
< first formulate a local optimality property, and then analyze it with duality
< theory and graph relaxation techniques.  Proof of the decentralized nature of
< the method is proved using group theory.
---
> \footnotetext{$^\dagger$ The main algorithm was first presented in the 2014 Robotics: Science and Systems conference~\citep{Liu-RSS-14}.}
> The work is extended from our recently proposed task-swap based anytime assignment
> method~\citep{liu-auro13}, which has a decentralized structure but may still entail multi-hop communication (global information).
> To eliminate the global communication constraint, we therefore further explore the decentralized structure  by carefully 
> analyzing and redefining the interactions between the search procedures that
> assess which tasks should be swapped.  Although the algorithm may produce
> suboptimal solutions, an inherent limitation arising from the fact that local
> information may be intrinsically inadequate, this new algorithm optimizes the
> search subject to the communication constraints and always produces the step
> with maximum convergence toward the optimal solution.
> Since local communication may impose limits that run against global
> optimality, we first formulate a local optimality property, and then 
> analyze it with duality theory and graph relaxation techniques. 
> Proof of the decentralized nature of the method is proved using group theory.
> 
> 
261,264c244,245
< hundreds, even thousands of robots). Specifically, a centralized algorithm can
< result in large computation/communication imbalance since the central
< controller is usually responsible for information collection and dissemination
< as well as data processing for the whole system. A heavy
---
> hundreds, even thousands of robots). Specifically, a centralized algorithm can be easily imbalanced in computation and communication since the central controller is usually responsible for information collection
> and dissemination as well as data processing for the whole system. A heavy
266c247
< in the low efficiency for the entire system. Also, a centralized coordination framework has poor robustness against failure owing to the dependence on the single central controller.  These drawbacks also apply to those semi-centralized architecture with a limited fixed number of central controllers.
---
> in the low efficiency for the entire system; Also, a centralized coordination framework has poor robustness against failure owing to the dependence on the single central controller.  These drawbacks also apply to those semi-centralized architecture with a limited fixed number of central controllers.
326,336c307,313
< Prior to this work, Liu and Shell proposed a task-swap based anytime assignment
< method~\citep{Liu-RSS-12} that is distributable, and yet optimal. It bridges
< the classical optimal assignment framework popular in operations research and
< the decentralized task allocation approaches developed and favored by
< roboticists.  Briefly, any stage of the algorithm naturally involves only a
< small subset of the robots and tasks, communication with other parts of the
< system may not even be required.  Yet, despite its decentralized nature, the
< method assumes that at each stage, the selected subset of robots can
< communicate with one another in some way, either via direct communication (when
< robots are within communication range, or when global broadcast communication
< exists) or a multi-hop network (if only local communication is available). 
---
> Prior to this proposed work, we proposed a task-swap based anytime assignment method~\citep{Liu-RSS-12} that is distributable, and yet optimal. It bridges the classical optimal
> assignment framework popular in operations research and the decentralized task allocation approaches developed and favored by roboticists. 
> Briefly, any stage of the algorithm naturally involves only a small subset of the robots and tasks, communication
> with other parts of the system may not even be required.  
> Yet, despite its decentralized nature, the method assumes that at each stage, the selected subset of robots can communicate with one another in some way, either via
> direct communication (when robots are within communication range, or when global
> broadcast communication exists) or a multi-hop network (if only local communication is available). 
1212c1189
< Thus far, the two aforementioned hurdles for decentralization\,---stage dependence and requirement of global communication---\,have been eliminated. 
---
> Thus far, the two aforementioned hurdles for decentralization ---\,stage dependence and requirement of global communication \,--- have been eliminated. 
1214c1191
< As a consequence, multiple swap loops can be searched concurrently and any robot is
---
> Consequently, multiple swap loops can be searched concurrently and any robot is
1218c1195
< Note that the robot that initiated the loop (the root of the search tree) does not need to explicitly communicate with the last robot on the tail in order to close the loop. This is because a loop closure can always be detected by the last robot on the chain and the task swaps can be done via backtracking along the loop.
---
> Note that, the robot that initiated the loop (the root of the search tree) does not need to explicitly communicate with the last robot on the tail in order to close the loop. This is because a loop closure can always be detected by the last robot on the chain and the task swaps can be done via backtracking along the loop.
1263c1240
< This means that a fully decentralized approach with the fewest interactions is desired. In other words, we prefer the local search processes to execute concurrently
---
> This means that, a fully decentralized approach with the fewest interactions is desired. In other words, we prefer the local search processes to execute concurrently
1265c1242
< We combine the permutation manipulations to explore the decentralized structure, and carefully examine interactions between the search procedures which assess the tasks to be swapped.
---
> We combine the permutation manipulations to explore the decentralized structure, and carefully examine interactions between the search procedures that assess which tasks should be swapped.
1282c1259
< In the decentralized implementation each robot carries out Algorithm~\ref{alg:relax} 
---
> In the decentralized implementation, each robot carries out Algorithm~\ref{alg:relax} 
1286,1290c1263,1264
< Finally, the algorithm does not need to use global information since the graph
< is only built from the network topology, however, the solution may be
< suboptimal because the network imposes constraints which confine the search so
< it will be an incomplete search of the global solution space.  Any resulting
< suboptimality reflects the constraints imposed by the network connectivity.
---
> Finally, the algorithm does not need to use global information since the graph is only built from the network topology, however, the solution may be suboptimal because the network imposes constraints which confine the search so it will be an incomplete search of the global solution space. 
> It is the constraints imposed by the network connectivity which are responsible for any resulting suboptimality:
1301c1275
< the relaxation runs to completeness, the largest cost reduction is found
---
> the relaxation runs to completeness the largest cost reduction is found
1323c1297
<   \caption{ Concurrent searching for swap loops. (a) The light-green circles represent robots and the smaller square dots denote tasks, where tasks can be mobile targets. Note that the longest edge on each loop is a virtual edge that closes the loop. In practice, a loop closure can always be detected by the last robot on the chain and the task swaps can be done via backtracking along the loop.  
---
>   \caption{ Concurrent searching for swap loops. (a) The light-green circles represent robots and the smaller square dots denote tasks, where tasks can be mobile targets. Note that, the longest edge on each loop is a virtual edge that closes the loop. In practice, a loop closure can always be detected by the last robot on the chain and the task swaps can be done via backtracking along the loop.  
1336c1310,1311
< Data were generated through a dispatching scenario: a group of robots in the plane
---
> 
> Data were generated via a dispatching scenario: a group of robots in the plane
1412c1387
< We next compared the convergence performance of the decentralized implementation (Algorithm~\ref{alg:dec}) with the recent 
---
> We next compared the convergence performance of the decentralized implementation (Algorithm~\ref{alg:dec}) with our recent 
1421c1396
< We define each time step as an interval that allows a message to be sent or received, and assume that a robot is able to duplicate messages when necessary and broadcast them to multiple receivers in a time step (similar to the communication strategy of {\sc Murdoch} architecture~\citep{Gerkey02sold}).
---
> We define each time step as an interval that allows a message to be sent or received, and assume that a robot is able to duplicate messages when necessary and broadcast them to multiple receivers in a time step (similar to the communication strategy of MURDOCH architecture~\citep{Gerkey02sold}).
1425,1427c1400,1402
< the optimal algorithm with stage dependence and global communication has a linear trend reaching the optimum, whereas the decentralized approaches with limited communication produces inferior results. 
< It should be emphasized, however, that without a multi-hop protocol the decentralized approach has limited information that can be shared; it is solving a more constrained optimization problem.
< Note also that owing to the local search being concurrent, the convergence rate of the decentralized is much faster than that of the centralized method. 
---
> the optimal algorithm with stage dependence and global communication has a linear trend toward reaching the optimality, whereas the decentralized approaches with limited communication produced inferior results. 
> It should be emphasized, however, that without a multi-hop protocol the decentralized approach is limited in what information can be shared; it is solving a more constrained optimization problem.
> We note that owing to the local search being concurrent, the convergence rate of the decentralized is much faster than that of the centralized method. 
1430c1405
< Then for the relaxation method, we enlarged the communication radius to $30m$, and observed that its convergence rate decreases whereas the solution (Relaxation+) is even closer to the optimum, which demonstrates Theorem~\ref{thm:comms-constraints}.
---
> Then for the relaxation method, we enlarged the communication radius to $30m$, and observed that its convergence rate decreases whereas the solution (Relaxation+) is even closer to the optimum, which validates Theorem~\ref{thm:comms-constraints}.
1438,1439c1413,1414
< convergence is quicker and the solution quality is improved. It also shows that
< the margin of improvement diminishes with increasing size, presumably reflecting the degree of parallelism intrinsic to the problem.
---
> convergence is quicker and the solution quality is better. It also shows that
> the margin of improvement diminishes as the number grows, presumably reflecting the degree of parallelism intrinsic to the problem.
1443c1418
< (ADOPT)~\citep{Modi06adopt} method, which also utilizes a search tree structure, was selected for evaluation.
---
> (ADOPT)~\citep{Modi06adopt} method, which also utilizes a search tree structure, was selected.
1445c1420
< ADOPT requires that a global search tree is constructed in which the agents each form tree nodes. 
---
> ADOPT requires that a global search tree is constructed wherein the agents each form tree nodes. 
1448c1423
< Then ADOPT controls the messages analogous to the branching technique in the Branch and Bound methods, but with special treatment and in a distributed fashion~\citep{Modi06adopt}.
---
> Then ADOPT controls the messages analogous to the branching technique in the Branch and Bound methods, but with special treatments and in a distributed fashion~\citep{Modi06adopt}.
1453c1428
< However, if the global tree is broken into multiple smaller trees ({e.g.}, owing to agent failures), then the performance deteriorates drastically. 
---
> However, if the global tree is broken into multiple smaller trees ({e.g.}, owing to the agent failures), then the performance deteriorates drastically. 

